Convexity and Optimization in Deficit Round Robin Scheduling for Delay-Constrained Systems

The Deficit Round Robin (DRR) scheduler is widely used in network systems for its simplicity and fairness. However, configuring its integer-valued parameters, known as quanta, to meet stringent delay constraints remains a significant challenge. This paper addresses this issue by demonstrating the convexity of the feasible parameter set for a two-flow DRR system under delay constraints. The analysis is then extended to n-flow systems, uncovering key structural properties that guide parameter selection. Additionally, we propose an optimization method to maximize the number of packets served in a round while satisfying delay constraints. The effectiveness of this approach is validated through numerical simulations, providing a practical framework for enhancing DRR scheduling. These findings offer valuable insights into resource allocation strategies for maintaining Quality of Service (QoS) standards in network slicing environments.

==> 4relatedwork.tex <==
\section{Related Work and Background}\label{RW}
DRR is a scheduling algorithm widely used in real-time systems and communication networks for its fairness and efficiency. Each queue in DRR is assigned a quantum, which defines the maximum amount of service allocated to the queue in each round. If the queue cannot fully utilize its quantum due to insufficient traffic or small task sizes, the unused portion—referred to as the residual deficit—is carried over to the next round. This mechanism ensures dynamic resource sharing, allowing idle capacity from underutilized queues to be reallocated to others.

DRR is particularly suited for time-sensitive networks, where strict bounds on worst-case delays are required. In such settings, flows with similar delay requirements are grouped into classes, with each class assigned to a DRR queue. The traffic from each flow is regulated by a leaky bucket or arrival curve constraint, which limits the amount of data sent within any given time interval.

While prior studies \cite{SEYED_ET_ALL_DRR_22, kanhere2002latency} have established worst-case delay bounds for DRR systems, these bounds do not directly address the challenge of configuring the quanta to simultaneously meet delay constraints for all flows. This is especially challenging in multi-flow systems with heterogeneous delay requirements, where determining the optimal vector of quanta that balances delay guarantees and scheduling efficiency remains an open problem with significant practical implications.
